An Overview of In-memory Processing with Emerging Non-volatile Memory for Data-intensive Applications

The conventional von Neumann architecture has been revealed as a major performance and energy bottleneck for rising data-intensive applications. %, due to the intensive data movements. The decade-old idea of leveraging in-memory processing to eliminate substantial data movements has returned and led extensive research activities. The effectiveness of in-memory processing heavily relies on memory scalability, which cannot be satisfied by traditional memory technologies. Emerging non-volatile memories (eNVMs) that pose appealing qualities such as excellent scaling and low energy consumption, on the other hand, have been heavily investigated and explored for realizing in-memory processing architecture. In this paper, we summarize the recent research progress in eNVM-based in-memory processing from various aspects, including the adopted memory technologies, locations of the in-memory processing in the system, supported arithmetics, as well as applied applications.

==> 2_0_Classifications.tex <==
\section{Design Overview}
\begin{figure}[b]
\centering
\vspace{-6pt}
\includegraphics[width=\columnwidth]{figure/fig_overview.pdf}	
\vspace{-12pt}
\caption{Processing locations and function types.} 
\label{fig:overview} 
\end{figure}
Table~\ref{tab:overview} presents a summary of the latest eNVM-based in-memory processing designs reviewed in this paper. 
Each of them is classified according to the following five main categories. 
%classification and overview of reviewed works in this paper. For each work, the below five main categories are classified:
\begin{itemize}
    \item \emph{Type -} The types of memory technologies adopted in these works: \textbf{STT-RAM, PCM} or \textbf{ReRAM}. Since the features of memories are different with each other, the selection of memory type determines the types of computation to some extent.
    \item \emph{Location -} Where is the memory located in the computing architecture: \textbf{cache, main memory} or \textbf{scratchpad}? 
    eNVMs can be used as storage and/or computing unit. 
    Some works treat eNVM only as \textbf{co-processor} while some designate its location in memory hierarchy too. %Some works designate the memory level where the memory located in hierarchy, while some treat eNVM as the \textbf{co-processor}. 
    \item \emph{Design Level -} The techniques in these works are carried out at different levels, such as \textbf{device, circuit} or \textbf{system}. 
    Some works proposed the novel writing method to perform calculations in memory cells~\cite{cassinerio2013logic,wright2013beyond,wright2011arithmetic,hosseini2015accumulation}. 
    Some techniques are achieved through the modifications of the readout or write circuits associated with memory arrays. 
    The system-level techniques would provide the interface and connection between the memory array and operation system so that the processing can be manipulated by applications.
    \item \emph{Functions -} The function types in these works can be divided into the following groups: \textbf{logic, arithmetic, associative, vector} and \textbf{matrix-vector multiplication (MVM)}. 
    A type of operation can be realized by different eNVMs, but the implementation details could vary significantly.
    \item \emph{Applications -} Most works provide advanced functions to support most data-intensive applications, which are grouped into~\textbf{generic}. 
    Some works carry out only the core operation in a number of applications such as~\textbf{encryption, database}, and \textbf{CNN}. 
    A few works complete simple and basic operations that are not designated to any targeted applications. 
    %Even though data-intensive applications play a crucial role to motivate in-memory processing, some works complete simple and basic operations and do not mention targeted applications. 
\end{itemize}



\begin{figure*}[t]
\centering
%\vspace{-12pt}
\includegraphics[width=.75\textwidth]{figure/fig_stt_bcnn_pan.pdf}	
\vspace{-9pt}
\caption{The execution flow, computing array, and multilevel STT-RAM cell for convolutional layers of Binary CNN in~\cite{pan2018multilevel}.} 
\label{fig:sttbcnn} 
\vspace{-12pt}
\end{figure*}

Figure~\ref{fig:overview} depicts a high-level view of the classifications based on the location of the in-memory processing in system (eNVM core, cache, scratchpad memory, or main memory) and the type of supported functions (bitwise logic, arithmetic, or associative).
% Table~\ref{tab:overview} further classifies the works based on the goal of the cache management technique and the essential approach, to allow the reader to see both similarities and differences between different works. 


==> 2_2_table_2.tex <==
\begin{table*}[t]
\caption{An Overview of In-memory Processing Designs}
\small
\vspace{-12pt}
\label{tab:overview}
% \begin{minipage}{\textwidth}
\begin{center}
\begin{tabular}{cc|c|c|ccc}
\toprule
%                 & SRAM & DRAM & STT-RAM & PCM & ReRAM\\\midrule
% Cell size(F$^2$) &   146   &      &    10     &  4-12   & 4 \\
% Write Endurance &      &      &    ~10$^15$     &  10$^8$-10$^11$   & 10$^8$-10$^10$ \\
% Speed(R/W)(ns)      &      &  /6.7    & <200$ps$/3-11$ns$&  15-20/20-25     & 6-8/20-30 \\
% Dynamic Energy (R/W)&      &  29.4mW/17.6mW$    &    /40$\muW$     &  /3$\pJ$   & 4 \\
% Leakage Power &      &      &         &     &  \\
      \multicolumn{2}{c|}{Works} & Types & Locations & Design Levels & Functions & Applications\\\midrule
Guo~\textit{et al.}~\cite{guo2010resistive} & 2010 &   \multirow{6}{*}{STT-RAM}   &  Cache    &    Circuit; System     &  Logic; Arithmetic &  Generic \\
AC-DIMM~\cite{guo2013ac} & 2013 &    &  Main Memory    &    Circuit; System     &  Associative &  Generic \\
% SPINDLE~\cite{ramasubramanian2014spindle} & 2014 &     &  Co-processor    &    Circuit; System     &  Logic &  Deep learning \\
Kang \textit{et al.}~\cite{kang2017memory} & 2017 &   &  -    &    Circuit     &  Logic &  Bitmap\\
STT-CiM~\cite{jain2018computing} & 2018 &     &  Scratchpad    &    Circuit; System     &  Logic; Addition; Vector &  Generic \\
HielM~\cite{parveen2018hielm} & 2018 &    &  -    &    Circuit; System  &  Logic & Encryption, Database\\
Pan \textit{et al.}~\cite{pan2018multilevel} & 2018 &     &  Co-processor    &    Circuit; System     &  Logic &  Binary CNN \\

\midrule
Cassinerio~\textit{et  al.}~\cite{cassinerio2013logic}& 2013 & \multirow{7}{*}{PCM}   &  -    &    Device  &  Logic &  - \\
Wright \textit{et al.}~\cite{wright2013beyond,wright2011arithmetic}& 2011, 2013 &    &  -    &    Device  &  Arithmetic &  - \\
Hosseini \textit{et al.}~\cite{hosseini2015accumulation}& 2015 &    &  -    &    Device  &  Arithmetic &  - \\
Pinatubo~\cite{li2016pinatubo} & 2015 &   & Main Memory    &  Circuit; System  &  Logic & Generic \\
Burr \textit{et al.}~\cite{burr2015experimental,burr2015large}& 2015 &   &  -    &    Circuit  &  MVM & DNN \\
Sebastian \textit{et al.}~\cite{sebastian2017temporal}& 2017 &   &  -    &    Circuit  &  MVM &  Unsupervised Learning \\
Le \textit{et al.}~\cite{le2017compressed,le2018mixed}& 2017, 2018 &   &  -    &    Circuit  &  MVM & Transfer Learning \\\midrule
MAGIC~\cite{kvatinsky2014magic}& 2014 & \multirow{6}{*}{ReRAM} & Co-processor & Circuit & Logic; Arithmetic & Adder \\ 
Bojnordi~\textit{et al.}\cite{bojnordi2016memristive}& 2016 & & Co-processor & System & MVM & Boltzmann machine \\
ISAAC~\cite{shafiee2016isaac} & 2016 & & Co-processor & System & MVM & CNN \\
PipeLayer~\cite{song2017pipelayer}& 2017 & & Co-processor & System & MVM & CNN \\
AtomLayer~\cite{qiao2018atomlayer}& 2018 & & Co-processor & System & MVM & CNN \\
GraphR~\cite{song2018graphr}& 2018 & & Co-processor & System & MVM & Graph \\

\bottomrule
\end{tabular}
\end{center}
%\bigskip
\footnotesize \emph{Note}: MVM -- Matrix-Vector Multiplication; DNN -- Deep Neural Network.
% \end{minipage}
\end{table*}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)
